BudgetLongformer: Can we Cheaply Pretrain a SotA Legal Language Model From Scratch?

Pretrained transformer models have achieved state-of-the-art results in many tasks and benchmarks recently. Many state-of-the-art Language Models (LMs), however, do not scale well above the threshold of 512 input tokens. In specialized domains though (such as legal, scientific or biomedical), models often need to process very long text (sometimes well above 10000 tokens). Even though many efficient transformers have been proposed (such as Longformer, BigBird or FNet), so far, only very few such efficient models are available for specialized domains. Additionally, since the pretraining process is extremely costly in general - but even more so as the sequence length increases - it is often only in reach of large research labs. One way of making pretraining cheaper is the Replaced Token Detection (RTD) task, by providing more signal during training, since the loss can be computed over all tokens. In this work, we train Longformer models with the efficient RTD task on legal data to showcase that pretraining efficient LMs is possible using much less compute. We evaluate the trained models on challenging summarization tasks requiring the model to summarize long texts to show to what extent the models can achieve good performance on downstream tasks. We find that both the small and base models outperform their baselines on the in-domain BillSum and out-of-domain PubMed tasks in their respective parameter range. We publish our code and models for research purposes.

==> sections/exluded_tokenizers_study.tex <==
%Study of tokenizers on BillSum Train Set
%mean num characters: 10272.54
%tokenizer                       type        vocab size  mean num tokens     character token ratio   
%bert-base-cased                 WP          29K         2023.09             5.078                   
%bert-base-uncased               WP          31K         1884.24             5.452                   
%albert-base-v2                  Unigram     30K         1935.68             5.307
%google/fnet-base                Unigram     32K         1947.43             5.275
%google/pegasus-large            Unigram     96K         1763.40             5.825                   
%microsoft/deberta-v3-base       Unigram     128K        1838.87             5.586
%ours                            BPE         64K         1909.23             5.380                   
%xlm-roberta-base                BPE         250K        2007.56             5.117                   
%allenai/longformer-base-4096    BPE         50K         3664.36             2.803
%gpt2                            BPE         50K         3664.36             2.803


==> summaries/billsum-1024-128_base_caselaw.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{21cm} }
    \toprule
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 5\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. AMENDMENT.

    Section 403 of the Social Security Act (42 U.S.C. 603) is amended 
by inserting after subsection (b) the following new subsection:
    ``(c)(1)(A) If the Secretary determines--
            ``(i) that a State is operating a general welfare 
        assistance program described in paragraph (3) during a calendar 
        quarter, or
            ``(ii) that more than 20 percent of the local governments 
        within a State that provide general welfare assistance are 
        operating programs described in paragraph (3) during a calendar 
        quarter,
the Secretary shall reduce by 50 percent the amount that such State 
would otherwise receive under subsection (a) with respect to 
expenditures made by such State during such quarter for the 
administration of the aid to families with dependent children program 
under this part.
    ``(B) If a State receives a reduced payment in a calendar quarter 
as a result of a determination by the Secretary under subparagraph 
(A)(ii)--
            ``(i) such State shall reduce for such quarter the payments 
        made to each State office administering the aid to families 
        with dependent children program which is located within the 
        jurisdiction of the local governments described in subparagraph 
        (A)(ii) by an amount equal to 50 percent of the of Federal 
        share of the administrative expenses of such office; and
            ``(ii) such State shall not, as a result of such reduced 
        payment, reduce for such quarter the payments made to any State 
        office administering the aid to families with dependent 
        children program which is not located within the jurisdiction 
        of the local governments described in subparagraph (A)(ii).
    ``(2) If the Secretary determines that any local government within 
a State that is not described in paragraph (1)(A) is operating a 
general welfare assistance program described in paragraph (3) during a 
calendar quarter, the State shall reduce for such quarter the payments 
made to any State office administering the aid to families with 
dependent children program which is located within the jurisdiction of 
such local government by an amount equal to 50 percent of the of 
Federal share of the administrative expenses of such office and such 
amount shall be paid by the State to the Secretary.
    ``(3) A general welfare assistance program described in this 
paragraph is a general welfare assistance pro... \\ 
 \midrule 
Gold & \tiny Amends part A (Aid to Families with Dependent Children) (AFDC) of title IV of the Social Security Act to require States to implement workfare programs for able-bodied residents on welfare aged 18 or over with no dependents in order for the State to maintain its current level of Federal funding for AFDC administrative expenses. \\ 
 \midrule 
Model & \small amends part a (temporary assistance for needy families) (tanf) of title iv of the social security act to direct the secretary of health and human services to reduce by 50 percent the amount that a state is operating a general welfare assistance program during a calendar quarter, or that more than 20 percent of the local governments within a state that provides general welfare assistance program during a calendar quarter.  requires such state to reduce by 50 percent the amount that such state would otherwise receive a reduced payment in a calendar quarter.  requires the secretary to report to congress on state and local participation rates. \\ 
 \midrule 
Metrics & Rouge1: 33.54, Rouge2: 13.84, RougeL: 23.6, RougeLsum: 26.09, Summary length (tokens): 120
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 25\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE; AMENDMENTS OF 1986 CODE.

    (a) Short Title.--This Act may be cited as the ``Natural Disaster 
Tax Relief Act of 1993''.
    (b) Amendment of 1986 Code.--Except as otherwise expressly 
provided, whenever in this Act an amendment or repeal is expressed in 
terms of an amendment to, or repeal of, a section or other provision, 
the reference shall be considered to be made to a section or other 
provision of the Internal Revenue Code of 1986.

SEC. 2. DISTRIBUTIONS FROM CERTAIN PLANS MAY BE USED WITHOUT PENALTY TO 
              REPLACE HOMES.

    (a) In General.--No additional tax shall be imposed under section 
72(t) of the Internal Revenue Code of 1986 on any distribution 
described in subsection (b) to the extent such distribution is used, 
within 60 days of the distribution, to pay qualified acquisition costs 
with respect to a principal residence of an eligible individual.
    (b) Distributions.--Subsection (a) shall apply to distributions--
            (1) from an individual retirement plan, or
            (2) from amounts attributable to employer contributions 
        made pursuant to elective deferrals described in subparagraph 
        (A) or (C) of section 402(g)(3) of the Internal Revenue Code of 
        1986 or section 501(c)(18)(D)(iii) of such Code.
    (c) Definitions and Special Rules.--
            (1) Eligible individual.--The term ``eligible individual'' 
        means an individual--
                    (A) who receives a distribution described in 
                subsection (b), or who is the spouse, child, or 
                grandchild of such individual, and
                    (B) whose principal residence was destroyed or 
                substantially damaged by Hurricane Andrew, Hurricane 
                Iniki, or Typhoon Omar.
            (2) Qualified acquisition costs.--The term ``qualified 
        acquisition costs'' means the costs of acquiring, constructing, 
        or reconstructing a residence. Such term includes any usual or 
        reasonable settlement, financing, or other closing costs.
            (3) Principal residence.--The term ``principal residence'' 
        has the same meaning as when used in section 1034 of such Code.
            (4) Distributions allowed.--A distribution to which 
        subsection (a) applies shall be treated as a distribution 
        allowed under section 401(k)(2)(B)(i) or 403(b)(11) of such 
        Code.
            (5) Transition.--In the case of any d... \\ 
 \midrule 
Gold & \tiny Natural Disaster Tax Relief Act of 1993 - Amends the Internal Revenue Code to allow penalty-free distributions from individual retirement plans to pay acquisition costs to replace a principal residence that was destroyed or substantially damaged by the disasters Hurricane Andrew, Hurricane Iniki, or Typhoon Omar. 
Allows a farmer who has income derived from the sale or exchange of crops grown in such disaster areas, to elect to defer such income for the next taxable year.  Provides a special rule for the self-employment tax. 
Requires the nonrecognition of gain of insurance proceeds for the contents of principal residences compulsorily or involuntarily converted as a result of a presidentially-declared disaster.  Allows insurance proceeds from personal property and real property to be lumped together into one common fund.  Extends the time to replace a principal residence so converted from two years to four years. 
Waives certain requirements with respect to low-income housing in areas damaged by the disasters Hurricane Andrew, Hurricane Iniki, or Typhoon Omar.  Waives the dollar limitation for home improvement loans through mortgage revenue bonds for residences in such disaster areas. \\ 
 \midrule 
Model & \small natural disaster tax relief act of 1993 - amends the internal revenue code to prohibit a distribution from an individual retirement account (ira) to the extent such distribution is used, within 60 days of such distribution, to pay qualified acquisition costs with respect to a principal residence of an eligible individual. 
allows distributions from an individual retirement plan (ira) or from amounts attributable to a principal residence if such sale was destroyed or substantially damaged by hurricane harvey, irma, or wilma. \\ 
 \midrule 
Metrics & Rouge1: 52.41, Rouge2: 27.03, RougeL: 35.29, RougeLsum: 51.34, Summary length (tokens): 97
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 75\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Telework Tax Incentive Act''.

SEC. 2. FINDINGS.

    The Congress finds as follows:
            (1) Federal, State, and local governments spend billions of 
        dollars annually on the Nation's transportation needs.
            (2) Congestion on the Nation's roads costs over 
        \$74,000,000,000 annually in lost work time, fuel consumption, 
        and costs of infrastructure and equipment repair.
            (3) On average on-road-vehicles contribute 30 percent of 
        nitrogen oxides emissions.
            (4) It is estimated that staying at home to work requires 3 
        times less energy consumption than commuting to work.
            (5) It was recently reported that if an identified 10 to 20 
        percent of commuters switched to teleworking, 1,800,000 tons of 
        regulated pollutants would be eliminated, 3,500,000,000 gallons 
        of gas would be saved, 3,100,000,000 hours of personal time 
        would be freed up, and maintenance and infrastructure costs 
        would decrease by \$500,000,000 annually because of reduced 
        congestion and reduced vehicle miles traveled.
            (6) The average American daily commute is 62 minutes for a 
        44-mile round-trip (a total of 6 days per year and 5,808 miles 
        per year).
            (7) The increase in work from 1969 to 1996, the increase in 
        hours mothers spend in paid work, combined with a shift toward 
        single-parent families resulted in families on average 
        experiencing a decrease of 22 hours a week (14 percent) in 
        parental time available outside of paid work they could spend 
        with their children.
            (8) Companies with teleworking programs have found that 
        teleworking can boost employee productivity 5 percent to 20 
        percent.
            (9) Today 60 percent of the workforce is involved in 
        information work (an increase of 43 percent since 1990) 
        allowing and encouraging decentralization of paid work to 
        occur.
            (10) In recent years, studies performed in the United 
        States have shown a marked expansion of teleworking, with an 
        estimate of 19,000,000 Americans teleworking by the year 2002, 
        5 times the amount in 1990.

SEC. 3. CREDIT FOR TELEWORKING.

    (a) In General.--Subpart B of part IV of subchapter A of chapter 1 
of the Internal Revenue Code of 1986 (relating to ... \\ 
 \midrule 
Gold & \tiny Telework Tax Incentive Act - Amends the Internal Revenue Code to allow a tax credit of up to \$500 annually for "qualified teleworking expenses." Defines such expenses. \\ 
 \midrule 
Model & \small teleworking tax incentive act - amends the internal revenue code to allow a tax credit of up to \$500 annually for teleworking expenses incurred by or on behalf of an individual teleworking arrangement, using electronic information and communication technologies, thereby reducing or eliminating the physical commute to and from the traditional location. limits the amount of such credit to \$500. \\ 
 \midrule 
Metrics & Rouge1: 54.12, Rouge2: 48.19, RougeL: 54.12, RougeLsum: 54.12, Summary length (tokens): 72
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 95\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Stop Iran From Smuggling Weapons to 
Terrorists Act''.

SEC. 2. AUTHORITY TO PROVIDE ASSISTANCE AND TRAINING TO INCREASE 
              MARITIME SECURITY AND DOMAIN AWARENESS OF FOREIGN 
              COUNTRIES BORDERING THE PERSIAN GULF, ARABIAN SEA, OR 
              MEDITERRANEAN SEA.

    (a) Purpose.--The purpose of this section is to authorize 
assistance and training to increase maritime security and domain 
awareness of foreign countries bordering the Persian Gulf, the Arabian 
Sea, or the Mediterranean Sea in order to deter and counter illicit 
smuggling and related maritime activity by Iran, including illicit 
Iranian weapons shipments.
    (b) Authority.--
            (1) In general.--To carry out the purpose of this section 
        as described in subsection (a), the Secretary of Defense, with 
        the concurrence of the Secretary of State, is authorized--
                    (A) to provide training to the national military or 
                other security forces of Israel, Bahrain, Saudi Arabia, 
                the United Arab Emirates, Oman, Kuwait, and Qatar that 
                have among their functional responsibilities maritime 
                security missions; and
                    (B) to provide training to ministry, agency, and 
                headquarters level organizations for such forces.
            (2) Designation.--The provision of assistance and training 
        under this section may be referred to as the ``Counter Iran 
        Maritime Initiative''.
    (c) Types of Training.--
            (1) Authorized elements of training.--Training provided 
        under subsection (b)(1)(A) may include the provision of de 
        minimis equipment, supplies, and small-scale military 
        construction.
            (2) Required elements of training.--Training provided under 
        subsection (b) shall include elements that promote the 
        following:
                    (A) Observance of and respect for human rights and 
                fundamental freedoms.
                    (B) Respect for legitimate civilian authority 
                within the country to which the assistance is provided.
    (d) Availability of Funds.--Of the amount authorized to be 
appropriated for fiscal year 2018 and available for operation and 
maintenance for Defense-wide activities, \$50,000,000 shall be available 
only for the provision of assistance and training under su... \\ 
 \midrule 
Gold & \tiny Stop Iran From Smuggling Weapons to Terrorists Act This bill authorizes the Department of Defense (DOD) to provide training to: (1) the national military or other security forces of Israel, Bahrain, Saudi Arabia, the United Arab Emirates, Oman, Kuwait, and Qatar that have among their functional responsibilities maritime security missions; and (2) ministry, agency, and headquarters level organizations for such forces.  Such assistance and training may be referred to as the Counter Iran Maritime Initiative. Such training: (1) may include the provision of de minimis equipment, supplies, and small-scale military construction; and (2) shall include the promotion of human rights and respect for legitimate civilian authority. It is the sense of Congress that DOD should seek payments from such countries to offset training costs. DOD shall negotiate a training cost-sharing agreement with a recipient country that covers at least 50\% of related costs. \\ 
 \midrule 
Model & \small stop iran from smuggling weapons to terrorists act this bill authorizes the department of defense (dod), with the concurrence of state, to: (1) provide training to the national military or other security forces of israel, france, saudi arabia, saudi arabia, and pakistan that have among their functional responsibilities maritime security missions; and (2) provide training to ministry, agency, and headquarters level organizations for such forces.  the provision of assistance and training shall include the provision of de minimis equipment, supplies, and small-scale military construction.  dod shall negotiate a cost-sharing agreement with a recipient country regarding: (1) initiation of \\ 
 \midrule 
Metrics & Rouge1: 76.77, Rouge2: 61.22, RougeL: 69.7, RougeLsum: 74.75, Summary length (tokens): 129
 \\ 

    \bottomrule
    \end{tabular}
}
\caption{Examples of the BillSum dataset using the model billsum-1024-128_base_caselaw}
\label{tab:examples_billsum-1024-128_base_caselaw}
\end{table*}


==> summaries/billsum-1024-128_base_diverse.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{21cm} }
    \toprule
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 5\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. NATIONAL GUARD SUPPORT FOR BORDER CONTROL ACTIVITIES.

    (a) Operation Jump Start.--
            (1) In general.--Not fewer than 6,000 National Guard 
        personnel shall continue to be deployed along the international 
        border between the United States and Mexico under Operation 
        Jump Start until the date on which the Federal Government has 
        achieved operational control of such border (as defined in 
        section 2(b) of the Secure Fence Act of 2006 (Public Law 109-
        367)).
            (2) Exemption.--National Guard personnel deployed pursuant 
        to paragraph (1) shall not be included in the calculation to 
        determine compliance with--
                    (A) limits on end strength; or
                    (B) limits on the number of National Guard personal 
                that may be placed on active duty for operational 
                support.
    (b) Support Authorized.--Chapter 1 of title 32, United States Code, 
is amended by inserting after section 112 the following:
``Sec. 112a. Border control activities
    ``(a) Funding Assistance.--The Secretary of Defense may provide 
funds to the Governor of a State who submits to the Secretary a State 
border control activities plan satisfying the requirements of 
subsection (c). Such funds shall be used for the following:
            ``(1) The pay, allowances, clothing, subsistence, 
        gratuities, travel, and related expenses, as authorized by 
        State law, of personnel of the National Guard of that State 
        used, while not in Federal service, for the purpose of border 
        control activities.
            ``(2) The operation and maintenance of the equipment and 
        facilities of the National Guard of that State used for the 
        purpose of border control activities.
            ``(3) The procurement of services and equipment, and the 
        leasing of equipment, for the National Guard of that State used 
        for the purpose of border control activities. However, the use 
        of such funds for the procurement of equipment may not exceed 
        \$5,000 per item, unless approval for procurement of equipment 
        in excess of that amount is granted in advance by the Secretary 
        of Defense.
    ``(b) Use of Personnel Performing Full-Time National Guard Duty.--
(1) Under regulations prescribed by the Secretary of Defense, personnel 
of the National Guard of a State may, in accordance with the State... \\ 
 \midrule 
Gold & \tiny Provides for continued National Guard support for border control activities along the U.S.- Mexico border under Operation Jump Start until operational control of such border has been achieved.

Authorizes the Secretary of Defense to provide funding to a state that submits to the Secretary of State a state border control activities plan that meets certain requirements. Limits the number of National Guard that may be so deployed. \\ 
 \midrule 
Model & \small (this measure has not been amended since it was passed by the senate on december 21, 2011. the summary of that version is repeated here.)

states that not fewer than six,000, national guard personnel shall continue to be deployed along the international border between the united states and mexico under operation jump start up to six,000 shall not be included in the annual calculation to determine compliance with: (1) limits on end strength or limits on the number of national guard personal that may be placed on active duty for operational support; and (2) the pay, allowances, and benefits of the national guard of a state shall \\ 
 \midrule 
Metrics & Rouge1: 46.33, Rouge2: 14.86, RougeL: 22.6, RougeLsum: 32.77, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 25\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``International Commerce Enhancement 
Act''.

SEC. 2. REFERENCES.

    Except as otherwise specifically provided in this Act, whenever in 
this Act an amendment or repeal is expressed as the amendment or repeal 
of a section or other provision, the reference shall be considered to 
be made to a section or other provision of the Arms Export Control Act 
(22 U.S.C. 2751 et seq.).

SEC. 3. FOREIGN AND NATIONAL SECURITY POLICY OBJECTIVES AND RESTRAINTS.

    (a) Value of Defense Articles and Services.--Section 3(d) (22 
U.S.C. 2753(d)) is amended in paragraphs (1) and (3)(A)--
            (1) by striking ``\$14,000,000'' each place it appears and 
        inserting ``\$25,000,000''; and
            (2) by striking ``\$50,000,000'' each place it appears and 
        inserting ``\$85,000,000''.
    (b) Transfers With Respect to NATO and Major Non-NATO Countries.--
Section 3(d) (22 U.S.C. 2753(d)) is amended--
            (1) in paragraph (2)--
                    (A) in subparagraph (A), by striking ``Except as 
                provided in subparagraph (B), unless'' and inserting 
                ``Unless''; and
                            (ii) in subparagraph (B) to read as 
                        follows:
    ``(B) Subparagraph (A) shall not apply in the case of a proposed 
transfer to the North Atlantic Treaty Organization, or any member 
country of such Organization, Japan, Australia, or New Zealand.''; and
                            (iii) in subparagraph (C), by striking ``or 
                        (B)''; and
            (2) in paragraph (3)--
                    (A) in the second sentence of subparagraph (A), by 
                striking ``shall be submitted'' and all that follows 
                through ``unless the President'' and inserting ``shall 
                be submitted at least 30 calendar days before such 
                consent is given in the case of a transfer to a country 
                other than a country which is a member of the North 
                Atlantic Treaty Organization, Japan, Australia, or New 
                Zealand, unless the President'';
                    (B) in the third sentence of subparagraph (A), by 
                striking ``(thus waiving the requirements of clause (i) 
                or (ii), as the case may be, and of subparagraph 
                (B))''; and
                    (C) in subparagraph (B)--
                            (i) by striking ... \\ 
 \midrule 
Gold & \tiny International Commerce Enhancement Act - Amends the Arms Export Control Act to increase threshold values of major defense equipment or defense articles or related training or other defense services whose transfer or lease to foreign countries would require a presidential certification to Congress. Exempts from specified congressional oversight requirements any such transfers to North Atlantic Treaty Organization (NATO) countries, Japan, Australia, or New Zealand. \\ 
 \midrule 
Model & \small international commerce enhancement act - amends the arms export control act to: (1) increase the amount of defense articles and services from \$10 million to \$10 million to \$10 million the value of defense articles and services (currently, \$10 million); (2) prohibit the transfer of defense articles or services to the north atlantic treaty organization (nato); and (3) prohibit the transfer of defense articles or services from the north atlantic treaty organization (nato) defense articles or services.

repeals the requirement that the transfer of defense articles or services from defense articles or services from the north atlantic treaty (nato) \\ 
 \midrule 
Metrics & Rouge1: 44.72, Rouge2: 21.38, RougeL: 34.78, RougeLsum: 38.51, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 75\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Family Education Reimbursement Act 
of 2005''.

SEC. 2. FAMILY EDUCATION REIMBURSEMENT ACCOUNTS.

    (a) Establishment.--The Secretary of Education, in consultation 
with the Secretary of Health and Human Services, shall--
            (1) establish a Family Education Reimbursement Account 
        Program under which, at the direction of the parent of each 
        displaced student who signs up under subsection (d), the 
        Secretary provides reimbursement to enable the student or 
        preschool-age child to attend the school or preschool program 
        of his or her parent's choice during the 2005-2006 school year;
            (2) of the amount available to carry out this section for 
        fiscal year 2006, use not more than one third of one percent of 
        such amount for administrative expenses, including outreach, 
        support services, and dissemination of information; and
            (3) contract with a nongovernmental entity to administer 
        and operate the program.
    (b) Reimbursement.--
            (1) In general.--In carrying out this section, the 
        Secretary--
                    (A) shall allow the parent of the participating 
                displaced student to select the school or preschool 
                program to be attended by the student during the 2005-
                2006 school year;
                    (B) at the direction of the parent, shall provide 
                reimbursement to that school or preschool program on a 
                quarterly basis; and
                    (C) in the case of a public school, may provide 
                such reimbursement to the appropriate local fiscal 
                agent for the school.
            (2) Amount.--In providing reimbursement under paragraph 
        (1), the Secretary shall--
                    (A) determine the amount of reimbursement to a 
                school or preschool program based on the number of 
                weeks during which the participating displaced student 
                attended the school or preschool program during the 
                preceding quarter;
                    (B) subject to subparagraph (C), provide the same 
                amount of reimbursement to each school and preschool 
                program for each week of attendance by one 
                participating displaced student;
                    (C) not provide reimbursement... \\ 
 \midrule 
Gold & \tiny Family Education Reimbursement Act of 2005 - Directs the Secretary of Education to establish a Family Education Reimbursement Account Program for families of students displaced by Hurricane Katrina or Hurricane Rita.

Provides for reimbursing parents for costs of such students or preschool-age children attending schools or preschool programs, chosen by the parents, during the 20052006 school year.

 Requires the Secretary to make a contract with a nongovernmental entity to administer and operate the program. \\ 
 \midrule 
Model & \small family education reimbursement act of 2005 - directs the secretary of education to establish a family education reimbursement account program under which, at the direction of the parent of each displaced student who signs up under the 2005- 2006 school year, the secretary of education shall: (1) provide reimbursement to the student or preschool child to attend the school or breakfast program of his or her parent's choice during the 2005- 2006- 2006 school year; (2) contract with a nongovernmental entity to administer and operate the program; and (3) contract with a nongovernmental entity to administer the program.

requires the secretary to develop and implement a web- \\ 
 \midrule 
Metrics & Rouge1: 63.74, Rouge2: 44.44, RougeL: 52.75, RougeLsum: 61.54, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 95\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Pharmaceutical Products Price Equity 
Act''.

SEC. 2. FINDINGS.

    The Congress finds the following:
            (1) Modern life enhancing and life sustaining drugs are the 
        products of decades of scientific research and practice.
            (2) The refining and production of products by American 
        pharmaceutical enterprises must be appropriately compensated.
            (3) The pricing of American pharmaceutical products varies 
        greatly from country to country with the corporate owners of 
        such products voluntarily assuming no losses by always selling 
        their products above the cost of production.
            (4) Considering the vital life and death nature of 
        pharmaceutical products, it is appropriate that the United 
        States Government, in harmony with other nations belonging to 
        the World Trade Organization, should engage in the reasonable 
        regulation of the prices of pharmaceutical products.

SEC. 3. REASONABLE LIMITS ON PROFITS OF PHARMACEUTICAL PRODUCTS.

    (a) Presidential Authority.--The President shall issue such orders 
and regulations, and establish such procedures and reporting 
requirements, as the President determines to be appropriate to ensure 
that no pharmaceutical product (as defined by the President in such 
regulation or order) is sold to any consumer in the United States at a 
price that is more than 6 percent above the average retail price at 
which such pharmaceutical product is sold in the 5 most industrialized, 
free-market countries, other than the United States, as determined by 
the President.
    (b) Delegation.--The President may delegate the performance of any 
function under this section to any officer of any Federal department or 
agency who has been appointed by the President, by and with the consent 
of the Senate.
    (c) Confidentiality of Information.--All information reported to or 
otherwise obtained by any person exercising any authority under this 
section which contains or relates to a trade secret or other matter 
referred to in section 1905 of title 18, United States Code, shall be 
considered confidential for purposes of that section, except that such 
information may be disclosed to any other officer or employee of the 
United States involved in carrying out this section solely for the 
purpose of carrying out, and enforcing compliance with, this section.
    (d) Subpoena Powe... \\ 
 \midrule 
Gold & \tiny Pharmaceutical Products Price Equity Act - Directs the President to issue orders and regulations, and establish procedures and reporting requirements, to ensure that no pharmaceutical product is sold to any consumer in the United States at a price that is more than six percent above the average retail price at which such pharmaceutical product is sold in the five most industrialized, free-market countries, other than the United States. Sets forth enforcement and civil liability provisions. \\ 
 \midrule 
Model & \small pharmaceutical products price equity act - directs the president to issue orders and regulations to ensure that no pharmaceutical product is sold to any consumer in the united states at a price more than six percent above the average retail price at which such product is sold in the five most industrialized, free-market countries, other than the united states. 
authorizes the president to delegate the performance of any such function to any federal department or agency who has been appointed by the president, by and with the consent of the senate, by and with the consent of the senate. \\ 
 \midrule 
Metrics & Rouge1: 70.11, Rouge2: 63.95, RougeL: 68.97, RougeLsum: 68.97, Summary length (tokens): 113
 \\ 

    \bottomrule
    \end{tabular}
}
\caption{Examples of the BillSum dataset using the model billsum-1024-128_base_diverse}
\label{tab:examples_billsum-1024-128_base_diverse}
\end{table*}


==> summaries/billsum-1024-128_small_caselaw.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{21cm} }
    \toprule
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 5\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as ``Cape Town Treaty Implementation Act of 
2004''.

SEC. 2. FINDINGS AND PURPOSE.

    (a) Findings.--Congress finds the following:
        (1) The Cape Town Treaty (as defined in section 44113 of title 
    49, United States Code) extends modern commercial laws for the 
    sale, finance, and lease of aircraft and aircraft engines to the 
    international arena in a manner consistent with United States law 
    and practice.
        (2) The Cape Town Treaty provides for internationally 
    established and recognized financing and leasing rights that will 
    provide greater security and commercial predictability in 
    connection with the financing and leasing of highly mobile assets, 
    such as aircraft and aircraft engines.
        (3) The legal and financing framework of the Cape Town Treaty 
    will provide substantial economic benefits to the aviation and 
    aerospace sectors, including the promotion of exports, and will 
    facilitate the acquisition of newer, safer aircraft around the 
    world.
        (4) Only technical changes to United States law and regulations 
    are required since the asset-based financing and leasing concepts 
    embodied in the Cape Town Treaty are already reflected in the 
    United States in the Uniform Commercial Code.
        (5) The new electronic registry system established under the 
    Cape Town Treaty will work in tandem with current aircraft document 
    recordation systems of the Federal Aviation Administration, which 
    have served United States industry well.
        (6) The United States Government was a leader in the 
    development of the Cape Town Treaty.
    (b) Purpose.--Accordingly, the purpose of this Act is to provide 
for the implementation of the Cape Town Treaty in the United States by 
making certain technical amendments to the provisions of chapter 441 of 
title 49, United States Code, directing the Federal Aviation 
Administration to complete the necessary rulemaking processes as 
expeditiously as possible, and clarifying the applicability of the 
Treaty during the rulemaking process.

SEC. 3. RECORDATION OF SECURITY INSTRUMENTS.

    (a) Establishment of System.--Section 44107(a) of title 49, United 
States Code, is amended--
        (1) in paragraph (2)(A) by striking ``750'' and inserting 
    ``550''; and
        (2) in paragraph (3) by striking ``clause (1) or (2) of this 
    subsection'' and inserting ``paragraph (1)... \\ 
 \midrule 
Gold & \tiny Cape Town Treaty Implementation Act of 2004 - Provides for implementation of the Convention on International Interests in Mobile Equipment, as modified by the Protocol to the Convention on International Interests in Mobile Equipment on Matters Specific to Aircraft Equipment, signed at Rome on May 9, 2003, or Cape Town Treaty (an electronic registry system for internationally established and recognized financing and leasing rights).

Amends Federal aviation law to revise requirements for the Federal Aviation Administration (FAA) system for recording conveyances that affect an interest in U.S. civil aircraft. Reduces from 750 to 550 the rated take-off horsepower (or equivalent) of any specifically identified aircraft engine with respect to which leases and security instruments are to be recorded in such system.

Designates the FAA Civil Aviation Registry as the United States Entry Point to the International Registry (established by the Cape Town Treaty) with respect to: (1) U.S. aircraft; (2) aircraft engines; and (3) any aircraft for which a U.S. identification number has been assigned, but only with regard to a notice filed under a system established by the Administrator for filing notices of prospective assignments and prospective international interests in, and prospective sales of, aircraft or aircraft engines under the Cape Town Treaty. Directs the FAA Administrator to establish such a system. Requires related documents to be filed for recordation within 60 days after such a notice is filed, or the notice, and any related registration with the International Registry, shall not be valid.

Makes any registration with the International Registry relating to an aircraft (other than aircraft engines) valid only if the person seeking the registration first files documents meeting the recordation requirements, and the U.S. Entry Point authorizes the registration.

Directs the Administrator to issue regulations which specify, at a minimum, the requirements for: (1) the registration of aircraft previously registered in a country in which the Cape Town Treaty is in effect; and (2) the cancellation of registration of a U.S. civil aircraft based on a request made in accordance with the Cape Town Treaty. \\ 
 \midrule 
Model & \small wall street convention implementation act of 2004 - amends the federal aviation administration (faa) to direct the federal aviation administration (faa) to establish a system for filing petitions to the international visitor center.

directs the administrator of the federal aviation administration (faa) to establish a system for filing fees and other requirements to be used by the united states for: (1) an aircraft for which a u.s. identification number has been assigned; and (2) an aircraft for which a u.s. identification number has been assigned is assigned.

requires the administrator to establish a system for filing fees and maximum filing fees. \\ 
 \midrule 
Metrics & Rouge1: 38.28, Rouge2: 13.53, RougeL: 22.01, RougeLsum: 33.49, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 25\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Manufacturing Modernization and 
Diversification Act of 2010''.

SEC. 2. DEFINITIONS.

    For purposes of this Act:
            (1) Bank.--The term ``bank'' means--
                    (A) an insured depository institution, as such term 
                is defined under section 3(c)(2) of the Federal Deposit 
                Insurance Act (12 U.S.C. 1813(c)(2)); and
                    (B) an insured credit union, as such term is 
                defined under section 101(7) of the Federal Credit 
                Union Act (12 U.S.C. 1752(7)).
            (2) Collateral support program.--The term ``Collateral 
        Support Program'' means a program described under section 4.
            (3) Loan participation program.--The term ``Loan 
        Participation Program'' means a program described under section 
        5.
            (4) Qualified manufacturer.--The term ``qualified 
        manufacturer'' means a business that is engaged in 
        manufacturing and--
                    (A) has less than \$50,000,000 in annual revenue; 
                and
                    (B) has less than \$50,000,000 in assets.
            (5) Revolving loan fund.--The term ``revolving loan fund'' 
        means the revolving loan fund established under section 3(d).
            (6) Secretary.--The term ``Secretary'' means the Secretary 
        of the Treasury.
            (7) SPV.--The term ``SPV'' means a special purpose vehicle 
        created by a State.
            (8) Termination date.--The term ``termination date'' means 
        the date that is the end of the 2-year period beginning on the 
        date the Secretary issues regulations pursuant to section 
        3(b)(4).

SEC. 3. FEDERAL LOAN PROGRAM TO SPVS.

    (a) In General.--The Secretary shall certify SPVs to take part in a 
program to carry out Collateral Support Programs and Loan Participation 
Programs for the benefit of qualified manufacturers (hereinafter in 
this section described as the ``loan program'').
    (b) Application Process.--
            (1) In general.--Each SPV wishing to participate in the 
        loan program shall submit an application to the Secretary, in 
        such form and manner as the Secretary may require, containing--
                    (A) a detailed proposal for the structure of the 
                Collateral Support Program the SPV proposes to carry 
                out, including what criteria the S... \\ 
 \midrule 
Gold & \tiny Manufacturing Modernization and Diversification Act of 2010 - Directs the Secretary of the Treasury to certify special purpose vehicles (SPVs) created by a state to take part in a program to carry out collateral support and loan participation programs for the benefit of qualified manufacturers (manufacturers with less than \$50 million in annual revenue and less than \$50 million in assets). Outlines SPV application requirements.

Allows, under the collateral support program, a qualified manufacturer that wishes to receive a bank loan but has insufficient collateral to ask the bank to seek collateral loan support from the SPV. Prohibits an SPV from providing more than \$20 million in collateral support to any one manufacturer. Requires manufacturers to be charged a fee for such support.

Allows, under the loan participation program, a qualified manufacturer that wishes to receive a bank loan but would not otherwise qualify for the loan to ask the bank to seek participation for such loan from the SPV. Prohibits an SPV from providing more than \$20 million in participation support to any one manufacturer. Requires manufacturers to be charged a fee for such support.

Requires: (1) periodic reports from such banks to participating SPVs; and (2) quarterly reports from the Secretary to Congress on participants in and impacts of the support and participation programs. \\ 
 \midrule 
Model & \small manufacturing modernization and retraining act of 2010 - directs the secretary of the treasury to certify annually to the national mortgage association (fannie mae) and the federal home loan mortgage corporation (freddie mac) programs (government sponsored enterprises or gses) that are engaged in manufacturing and have less than \$5 billion in annual revenue, and have less than \$5 billion.

directs the secretary to: (1) certify annually to the secretary that an application for such a loan participation is made available; and (2) establish an advisory process for making such a program.

amends the internal revenue code to: (1) allow a tax \\ 
 \midrule 
Metrics & Rouge1: 43.6, Rouge2: 18.18, RougeL: 32.23, RougeLsum: 37.91, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 75\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Higher Education Family Opportunity 
Act of 1998''.

SEC. 2. DEDUCTION FOR POSTSECONDARY TUITION AND RELATED EXPENSES IN 
              LIEU OF HOPE AND LIFETIME LEARNING CREDIT.

    (a) In General.--Part VII of subchapter B of chapter 1 of the 
Internal Revenue Code of 1986 (relating to additional itemized 
deductions for individuals) is amended by redesignating section 222 as 
section 223 and by inserting after section 221 the following new 
section:

``SEC. 222. DEDUCTION FOR POSTSECONDARY TUITION AND RELATED EXPENSES IN 
              LIEU OF HOPE AND LIFETIME LEARNING CREDIT.

    ``(a) Allowance of Deduction.--In the case of an individual, there 
shall be allowed as a deduction for the taxable year an amount equal to 
the qualified tuition and related expenses paid or incurred by such 
individual.
    ``(b) Limitation.--
            ``(1) In general.--The amount allowable as a deduction 
        under subsection (a) for a taxable year shall not exceed the 
        deductible limit for each eligible student.
            ``(2) Deductible limit.--For purposes of paragraph (1), the 
        deductible limit for a taxable year shall be determined in 
        accordance with the following table:

``Taxable years beginning                                              
  in calendar year:                                   Deductible limit:
        1999................................................... \$5,000 
        2000................................................... \$5,500 
        2001................................................... \$6,000 
        2002................................................... \$6,500 
        2003................................................... \$7,000 
        2004................................................... \$7,500 
        2005................................................... \$8,000 
        2006................................................... \$8,500 
        2007................................................... \$9,000 
        2008................................................... \$9,500 
        2009 and thereafter....................................\$10,000.
    ``(c) Qualified Tuition and Related Expenses; Eligible Student.--
The terms `qualified tuition and related expenses' and `eligible 
student' shall have the same meanings given to such terms by section 
25A.
    ``(d) Applicable Rules.--For purposes of this section, rules 
similar to... \\ 
 \midrule 
Gold & \tiny Higher Education Family Opportunity Act of 1998 - Amends the Internal Revenue Code to permit a deduction for qualified tuition and related expenses in lieu of the Hope and Lifetime Learning credits. Sets the deductible limit at \$5,000 for 1999 and increases such limit by \$500 annually until it reaches \$10,000 for years 2009 and thereafter. \\ 
 \midrule 
Model & \small higher education family opportunity act of 1998 - amends the internal revenue code to allow individual taxpayers a deduction from gross income for higher education tuition and related expenses up to \$2,000. \\ 
 \midrule 
Metrics & Rouge1: 47.19, Rouge2: 36.78, RougeL: 47.19, RougeLsum: 47.19, Summary length (tokens): 39
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 95\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Environmental Export Promotion Act 
of 1994''.

SEC. 2. PROMOTION OF UNITED STATES ENVIRONMENTAL EXPORTS.

    (a) Environmental Technologies Trade Advisory Committee.--Section 
2313 of the Export Enhancement Act of 1988 (15 U.S.C. 4728) is 
amended--
            (1) by striking subsection (d);
            (2) by redesignating subsection (c) as subsection (e); and
            (3) by inserting after subsection (b) the following new 
        subsections:
    ``(c) Environmental Technologies Trade Advisory Committee.--
            ``(1) Establishment and purpose.--The Secretary, in 
        carrying out the duties of the chairperson of the TPCC, shall 
        establish the Environmental Technologies Trade Advisory 
        Committee (hereafter in this section referred to as the 
        `Committee'). The purpose of the Committee shall be to provide 
        advice and guidance to the Working Group in the development and 
        administration of programs to expand United States exports of 
        environmental technologies, goods, and services.
            ``(2) Membership.--
                    ``(A) In general.--The members of the Committee 
                shall be drawn from representatives of--
                            ``(i) environmental businesses, including 
                        small businesses;
                            ``(ii) trade associations in the 
                        environmental sector;
                            ``(iii) private sector organizations 
                        involved in the promotion of environmental 
                        exports;
                            ``(iv) the States (as defined in section 
                        2301(j)(5)) and associations representing the 
                        States; and
                            ``(v) other appropriate interested members 
                        of the public.
                    ``(B) Committee composition.--The Secretary shall 
                appoint as members of the Committee no fewer than 1 
                individual under each of clauses (i) through (v) of 
                subparagraph (A).
    ``(d) Export Plans for Priority Countries.--
            ``(1) Priority country identification.--The Working Group, 
        in consultation with the Committee, shall annually assess which 
        foreign countries have markets with the greatest potential for 
        the export of United States ... \\ 
 \midrule 
Gold & \tiny Environmental Export Promotion Act of 1994 - Amends the Export Enhancement Act of 1988 to direct the Secretary of Commerce to establish the Environmental Technologies Trade Advisory Committee to advise and guide the Environmental Trade Promotion Working Group in the development and administration of programs to expand U.S. exports of environmental technologies, goods, and services. 
Requires the Working Group to assess annually which foreign countries have markets with the greatest potential for such exports, and select five of them as priority countries for the application of U.S. Government export promotion resources.  Requires the Working Group to create annual plans for each priority country, detailing ways to increase U.S. environmental exports to such country. 
Directs the Secretary to assign a specialist in environmental technologies to the office of the United States and Foreign Commercial Service in each of the five priority countries, and authorize similar assignments in any countries that are promising markets for such exports.  Specifies the duties of such specialists. 
Requires the Secretary to establish:  (1) a mechanism to give environmental technology and international environmental marketplace training to Commercial Service Officers assigned to one-stop shops and to district offices in districts with large numbers of environmental businesses; and (2) ensure that such officers receive appropriate training under such mechanism. 
Directs the Trade Promotion Coordinating Committee (TPCC) to establish not less than one international regional environmental initiative to coordinate Federal activities to build environmental partnerships between the United States and the geographic region outside the United States for which such an initiative is established. Specifies TPCC activities in carrying out such initiative. 
Directs the Working Group to maintain an environmental technologies project advocacy calendar, updated quarterly, identifying and providing information on significant project opportunities for U.S. environmental businesses in foreign markets and trade promotion events. 
Authorizes the Secretary to provide matching funds for the establishment in the United States of regional environmental business and technology cooperation centers that will draw upon the expertise of the private sector, institutions of higher education, and existing Federal programs to provide export promotion assistance related to environmental technologies, goods, and services. \\ 
 \midrule 
Model & \small environmental export promotion act of 1994 - amends the export enhancement act of 1988 to direct the secretary of commerce to establish the environmental technologies trade advisory committee to provide advice and guidance to the working group in the development and administration of programs to expand u.s. export promotion resources. 
requires the working group to:  (1) identify foreign countries with the greatest potential for the application of environmental technologies, goods, and services; (2) list specific actions to be taken by the working group to increase u.s. export promotion and export promotion resources related to environmental imports; and (3) list specific actions to be taken by \\ 
 \midrule 
Metrics & Rouge1: 73.15, Rouge2: 61.68, RougeL: 61.11, RougeLsum: 67.59, Summary length (tokens): 129
 \\ 

    \bottomrule
    \end{tabular}
}
\caption{Examples of the BillSum dataset using the model billsum-1024-128_small_caselaw}
\label{tab:examples_billsum-1024-128_small_caselaw}
\end{table*}


==> summaries/billsum-1024-128_small_diverse.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{21cm} }
    \toprule
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 5\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Child Citizenship Act of 2000''.

   TITLE I--CITIZENSHIP FOR CERTAIN CHILDREN BORN OUTSIDE THE UNITED 
                                 STATES

SEC. 101. AUTOMATIC ACQUISITION OF CITIZENSHIP FOR CERTAIN CHILDREN 
              BORN OUTSIDE THE UNITED STATES.

    (a) In General.--Section 320 of the Immigration and Nationality Act 
(8 U.S.C. 1431) is amended to read as follows:

 ``children born outside the united states and residing permanently in 
  the united states; conditions under which citizenship automatically 
                                acquired

    ``Sec. 320. (a) A child born outside of the United States 
automatically becomes a citizen of the United States when all of the 
following conditions have been fulfilled:
        ``(1) At least one parent of the child is a citizen of the 
    United States, whether by birth or naturalization.
        ``(2) The child is under the age of eighteen years.
        ``(3) The child is residing in the United States in the legal 
    and physical custody of the citizen parent pursuant to a lawful 
    admission for permanent residence.
    ``(b) Subsection (a) shall apply to a child adopted by a United 
States citizen parent if the child satisfies the requirements 
applicable to adopted children under section 101(b)(1).''.
    (b) Clerical Amendment.--The table of sections of such Act is 
amended by striking the item relating to section 320 and inserting the 
following:
``Sec. 320. Children born outside the United States and residing 
          permanently in the United States; conditions under which 
          citizenship automatically acquired.''.

SEC. 102. ACQUISITION OF CERTIFICATE OF CITIZENSHIP FOR CERTAIN 
              CHILDREN BORN OUTSIDE THE UNITED STATES.

    (a) In General.--Section 322 of the Immigration and Nationality Act 
(8 U.S.C. 1433) is amended to read as follows:

``children born and residing outside the united states; conditions for 
                  acquiring certificate of citizenship

    ``Sec. 322. (a) A parent who is a citizen of the United States may 
apply for naturalization on behalf of a child born outside of the 
United States who has not acquired citizenship automatically under 
section 320. The Attorney General shall issue a certificate of 
citizenship to such parent upon proof, to the satisfaction of the 
Attorney General, that the following conditions have been fulfilled:
        ``(1) At least one parent ... \\ 
 \midrule 
Gold & \tiny Provides for issuance of a certificate of naturalization for a child born outside of the United States when the following conditions are met: (1) at least one parent is a U.S. citizen who has been present in the United States for not less than five years, at least two of which were after having attained the age of 14, or who has a citizen parent meeting such requirements; (2) the child is under 18 years old; and (3) the child is residing outside the United States in the legal and physical custody of the citizen parent, is temporarily and lawfully present in the United States, and is maintaining such lawful status. Applies such provision to an adopted child meeting certain definitional requirements who is adopted by a U.S. citizen parent.
Title II: Protections for Certain Aliens Voting Based on Reasonable Belief of Citizenship
 - Amends the Immigration and Nationality Act respecting unlawful voting or false U.S. citizenship claims by permanent resident aliens under 16 years old having natural or adoptive U.S. citizen parents, to provide exceptions from certain provisions regarding deportability, moral character, inadmissability or related criminal penalties. \\ 
 \midrule 
Model & \small table of contents: 
     title i: citizenship for certain 
     title ii:  immigration and naturalization provisions 
title i: citizenship for certain children born outside the united states
 - amends the immigration and nationality act (ina) to revise naturalization requirements with respect to child born outside the united states. 
(sec. 102) amends the immigration and nationality act to revise requirements with respect to:  (1) naturalization as a citizen of the united states; (2) naturalization of a u.s. citizen; (3) citizenship; (4) citizenship; (5) naturalization service; and (6) \\ 
 \midrule 
Metrics & Rouge1: 35.9, Rouge2: 15.54, RougeL: 22.56, RougeLsum: 20.51, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 25\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Effective Terrorists Prosecution Act 
of 2006''.

SEC. 2. DEFINITION OF UNLAWFUL ENEMY COMBATANT.

    Paragraph (1) of section 948a of title 10, United States Code (as 
enacted by the Military Commissions Act of 2006 (Public Law 109-366)), 
is amended to read as follows:
            ``(1) Unlawful enemy combatant.--The term `unlawful enemy 
        combatant' means an individual who directly participates in 
        hostilities as part of an armed conflict against the United 
        States who is not a lawful enemy combatant. The term is used 
        solely to designate individuals triable by military commission 
        under this chapter.''.

SEC. 3. DETERMINATION OF UNLAWFUL ENEMY COMBATANT STATUS BY COMBATANT 
              STATUS REVIEW TRIBUNAL NOT DISPOSITIVE FOR PURPOSES OF 
              JURISDICTION OF MILITARY COMMISSIONS.

    Section 948d of title 10, United States Code (as enacted by the 
Military Commissions Act of 2006 (Public Law 109-366)), is amended--
            (1) by striking subsection (c); and
            (2) by redesignating subsection (d) as subsection (c).

SEC. 4. EXCLUSION FROM TRIAL BY MILITARY COMMISSION OF STATEMENTS 
              OBTAINED BY COERCION.

    Section 948r of title 10, United States Code (as enacted by the 
Military Commissions Act of 2006 (Public Law 109-366)), is amended by 
striking subsections (c) and (d) and inserting the following new 
subsection (c):
    ``(c) Exclusion of Statements Obtained by Coercion.--A statement 
obtained by use of coercion shall not be admissible in a military 
commission under this chapter, except against a person accused of 
coercion as evidence that the statement was made.''.

SEC. 5. DISCRETION OF MILITARY JUDGE TO EXCLUDE HEARSAY EVIDENCE 
              DETERMINED TO BE UNRELIABLE OR LACKING IN PROBATIVE 
              VALUE.

    Section 949a(b)(2)(E)(ii) of title 10, United States Code (as 
enacted by the Military Commissions Act of 2006 (Public Law 109-366)), 
is amended by striking ``if the party opposing the admission of the 
evidence demonstrates that the evidence is unreliable or lacking in 
probative value'' and inserting ``if the military judge determines, 
upon motion by counsel, that the evidence is unreliable or lacking in 
probative value''.

SEC. 6. DISCRETION OF MILITARY JUDGE TO TAKE CERTAIN ACTIONS IN EVENT 
              THAT A SUBSTITUTE FOR CLASSIFIED EXCULPATORY EVIDENCE IS 
              INS... \\ 
 \midrule 
Gold & \tiny Effective Terrorists Prosecution Act of 2006 - Amends federal armed forces provisions enacted by the Military Commissions Act of 2006 to, among other things: (1) exclude from military commission (commission) trials statements obtained by coercion; (2) allow a commission military judge to exclude hearsay evidence determined to be unreliable or lacking in probative value; (3) provide for review of commission decisions by the U.S. Court of Appeals for the Armed Forces rather than the Court of Military Commission Review; (4) revise generally provisions concerning the implementation of treaty obligations with respect to the U.S. prosecution of enemy combatants; (5) restore habeas corpus rights for individuals detained by the United States; and (6) provide for expedited judicial review of provisions of the Military Commissions Act of 2006. \\ 
 \midrule 
Model & \small effective terrorists prosecution act of 2006 - amends federal armed forces law to revise the definition of " unlawful enemy combatant" to include an individual who directly participated in hostilities as part of an armed conflict against the united states who is not a lawful enemy combatant.

amends the military pay reform and reform act of 2006 to provide that a complaint obtained by mail or the military court of appeals for the u.s. military court of appeals for the armed forces who is not a lawful enemy combatant.

directs the u.s. military department of defense to review the record in each case, except against a person aggrieved by prosecution or \\ 
 \midrule 
Metrics & Rouge1: 51.64, Rouge2: 24.64, RougeL: 33.8, RougeLsum: 37.56, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 75\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``Census Address List Improvement Act 
of 1994''.
SEC. 2. ADDRESS INFORMATION REVIEWED BY LOCAL GOVERNMENTS.
    (a) In General.--Chapter 1 of title 13, United States Code, is 
amended by adding after section 15 the following new section:
``Sec. 16. Address information reviewed by States and local governments
    ``(a) The Secretary, to assist efforts to ensure the accuracy of 
censuses and surveys under this title, shall--
        ``(1) publish standards defining the content and structure of 
    address information which States and local units of general purpose 
    government may submit to the Secretary to be used in developing a 
    national address list;
        ``(2)(A) develop and publish a timetable for the Bureau to 
    receive, review, and respond to submissions of information under 
    paragraph (1) before the decennial census date; and
        ``(B) provide for a response by the Bureau with respect to such 
    submissions in which the Bureau specifies its determinations 
    regarding such information and the reasons for such determinations; 
    and
        ``(3) be subject to the review process developed under section 
    3 of the Census Address List Improvement Act of 1994 relating to 
    responses pursuant to paragraph (2).
    ``(b)(1) The Secretary--
        ``(A) shall provide officials who are designated as census 
    liaisons by a local unit of general purpose government with access 
    to census address information for the purpose of verifying the 
    accuracy of the address information of the Bureau for census and 
    survey purposes; and
        ``(B) together with such access, should provide an explanation 
    of duties and obligations under this title.
    ``(2) Access under paragraph (1) shall be limited to address 
information concerning addresses within the local unit of general 
purpose government represented by the census liaison or an adjacent 
local unit of general purpose government.
    ``(3) The Bureau should respond to each recommendation made by a 
census liaison concerning the accuracy of address information, 
including the determination (and reasons therefor) of the Bureau 
regarding each such recommendation.
    ``(4) For the purposes of paragraph (1), in a case in which a local 
unit of general purpose government is within another local unit of 
general purpose government and is not independent of the enclosing 
unit, the census liaison shall be ... \\ 
 \midrule 
Gold & \tiny Census Address List Improvement Act of 1994 - Directs the Secretary of Commerce to:  (1) publish standards defining the content and structure of address information which States and local governments may submit to the Secretary to be used in developing a national address list; (2) develop and publish a timetable for the Bureau of the Census to receive, review, and respond to the submitted information before the decennial census date; (3) provide for a response by the Bureau that specifies its determinations regarding such information and the reasons for such determinations; and (4) be subject to the review process developed under this Act relating to such responses. 
Directs the Secretary to provide officials who are designated as census liaisons by local governments with access to census address information for the purpose of verifying the accuracy of the Bureau's address information for census and survey purposes and together with such access, provide an explanation of duties and obligations under this Act. 
Limits such access to the addresses within the local government represented by the census liaison or an adjacent local government. 
Requires the Bureau to respond to each recommendation made by a census liaison concerning the accuracy of address information, including the determination (and reasons therefor) of the Bureau regarding each such recommendation. 
Prohibits a census liaison from using information made available under this Act for purposes other than the purposes specified in this Act. 
Makes provisions that require, with exceptions, that such information be treated as confidential applicable to local government census liaisons.  Imposes a fine and up to five years' imprisonment on whoever being or having been a census liaison wrongfully discloses such information. 
Requires:  (1)  the Administrator of the Office of Information and Regulatory Affairs, acting through the Chief Statistician, to develop an appeals process for those States and local governments which desire to appeal determinations of the Bureau; and (2)  the Postal Service to provide to the Secretary for use by the Bureau such address, address- related, and point of postal delivery information, including postal delivery codes, determined by the Secretary to be appropriate for any census or survey being conducted by the Bureau. \\ 
 \midrule 
Model & \small census address list improvement act of 1994 - directs the secretary of transportation to:  (1) publish standards amending the content and structure of address information which states and local governments may submit to the secretary to the secretary to the secretary for such a national address list; (2) provide for a response by a census liaison with respect to such reports; and (3) provide for a response by a census liaison with respect to such reports. 
requires the secretary to:  (1) provide officials who are designated as census liaison with access to census information; and (2) report annually to the congressional committees on the accuracy of \\ 
 \midrule 
Metrics & Rouge1: 62.26, Rouge2: 41.9, RougeL: 50.0, RougeLsum: 52.83, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 95\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny SECTION 1. SHORT TITLE.

    This Act may be cited as the ``National Geologic Mapping 
Reauthorization Act of 1996''.

SEC. 2. FINDINGS.

    Congress finds that--
            (1) in enacting the National Geologic Mapping Act of 1992 
        (43 U.S.C. 31a et seq.), Congress found, among other things, 
        that--
                    (A) during the 2 decades preceding enactment of 
                that Act, the production of geologic maps had been 
                drastically curtailed;
                    (B) geologic maps are the primary data base for 
                virtually all applied and basic earth-science 
                investigations;
                    (C) Federal agencies, State and local governments, 
                private industry, and the general public depend on the 
                information provided by geologic maps to determine the 
                extent of potential environmental damage before 
                embarking on projects that could lead to preventable, 
                costly environmental problems or litigation;
                    (D) the lack of proper geologic maps has led to the 
                poor design of such structures as dams and waste-
                disposal facilities;
                    (E) geologic maps have proven indispensable in the 
                search for needed fossil fuel and mineral resources; 
                and
                    (F) a comprehensive nationwide program of geologic 
                mapping is required in order to systematically build 
                the Nation's geologic-map data base at a pace that 
                responds to increasing demand;
            (2) the geologic mapping program called for by that Act has 
        not been fully implemented; and
            (3) it is time for this important program to be fully 
        implemented.

SEC. 3. REAUTHORIZATION AND AMENDMENT.

    (a) Definitions.--Section 3 of the National Geologic Mapping Act of 
1992 (43 U.S.C. 31b) is amended--
            (1) by striking ``As used in this Act:'' and inserting ``In 
        this Act:'';
            (2) by redesignating paragraphs (2), (3), (4), and (5) as 
        paragraphs (3), (4), (5), and (6), respectively;
            (3) by inserting after paragraph (1) the following:
            ``(2) Association.--The term `Association' means the 
        Association of American State Geologists.''; and
            (4) in each paragraph that does not have a heading, by 
      ... \\ 
 \midrule 
Gold & \tiny National Geologic Mapping Reauthorization Act of 1996 - Amends the National Geologic Mapping Act of 1992 to establish a national cooperative geologic mapping program between the U.S. Geological Survey and State geological surveys. 
Establishes a geologic mapping advisory committee to advise the Director of the U.S. Geological Survey on planning and implementation of the geological mapping program. 
Authorizes appropriations. \\ 
 \midrule 
Model & \small national geologic mapping reauthorization act of 1996 - amends the national geologic mapping act of 1992 to establish a national cooperative geologic mapping program within the united states geological survey (usgs) to be administered and administered through the association. 
establishes a national cooperative geologic mapping program between the united states geological survey and the association.  authorizes appropriations. \\ 
 \midrule 
Metrics & Rouge1: 74.14, Rouge2: 56.14, RougeL: 65.52, RougeLsum: 67.24, Summary length (tokens): 69
 \\ 

    \bottomrule
    \end{tabular}
}
\caption{Examples of the BillSum dataset using the model billsum-1024-128_small_diverse}
\label{tab:examples_billsum-1024-128_small_diverse}
\end{table*}


==> summaries/pubmed-1024-128_base_diverse.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{21cm} }
    \toprule
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 5\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny cdnas 
  containing the sequence of human wt - ftl and human mutant 
  ftl498499instc were introduced into the pet-28a(+ ) expression 
  vector ( novagen , emd chemicals inc . ) . 
 the cdnas were cloned between the bamhi 
  and xhoi sites , downstream from and in - frame with the sequence encoding an 
  n - terminal his6 tag . to eliminate the his6 tag ( included 
  in the expression vector ) , 
 the sequence of the vector was modified by 
  introducing the recognition sequence for cleavage by factor xa before the 
  coding sequence of the ferritin genes . 
 pcr amplification of the ferritin cdnas 
  was performed using the upstream primer f1 5-tgg atc cat cga agg 
  tcg tat gag ctc cca gat t-3 and the downstream primer r1 
  5-tta tgc ctc gag ccc tat tac ttt gca agg-3. f1 contains the 
  factor xa sequence ( underlined ) . 
 pet-28a(+ ) carrying wt - ftl and mt - ftl cdnas 
  was transformed into bl21 ( de3 ) escherichia coli ( invitrogen ) . 
 transformed cells were grown in luria broth medium ( lb ) containing 30 g / ml 
  kanamycin ( invitrogen ) at 37 c up to an absorbance of 0.91.0 at 
  600 nm . 
 bacteria were induced to overexpress recombinant proteins by adding 1 
  mm isopropyl thio--d - galactopyranoside ( icn 
  biotechnologies ) for 12 h at 25 c . 
 purification of recombinant wt- and mt - ftl 
  homopolymers  cells were harvested by centrifugation and frozen at 
  -80 c . 
 the cell pellets were suspended in 50 mm sodium 
  phosphate , 500 mm nacl ( ph 7.4 ) , 1 mg / ml lysozyme , and a protease 
  inhibitor mixture ( complete , roche applied science ) for 30 min . 
 bacteria were 
  disrupted by sonication , and the insoluble material was removed by 
  centrifugation at 21,000  g for 30 min . 
 the soluble fraction 
  was purified by nickel iminodiacetic acid affinity chromatography using an 
  akta purifier system ( ge healthcare ) . 
 purified protein was eluted with 250 
  mm imidazole in 50 mm sodium phosphate ( ph 7.4 ) , 0.5 
  m nacl . 
 recombinant proteins were diluted with 50 mm 
  tris and 10\% glycerol ( v / v ) down to an absorbance of 0.5 at 280 nm , and 
  ferritins were cleaved from the his tag by digestion with factor xa protease 
  ( ge healthcare ) ( 5 units / mg of protein ) . after being dialyzed against 50 
  mm tris , ph 8.0 , for 18 h , proteins were further purified by anion 
  exchange chromatography ( mono q ) using a linear nacl elution gradient in 50 
  mm tris ( ph 8) . 
 peak fractions were 95\% pure based on s... \\ 
 \midrule 
Gold & \tiny nucleotide insertions in the ferritin light chain ( ftl ) polypeptide gene 
  cause hereditary ferritinopathy , a neurodegenerative disease characterized by 
  abnormal accumulation of ferritin and iron in the central nervous system . here 
 we describe for the first time the protein structure and iron storage function 
  of the ftl mutant p.phe167serfsx26 ( mt - ftl ) , which has a c terminus 
  altered in sequence and extended in length . 
 mt - ftl polypeptides assembled 
  spontaneously into soluble , spherical 24-mers that were ultrastructurally 
  indistinguishable from those of the wild type . 
 far - uv cd showed a decrease in 
  -helical content , and 8-anilino-1-naphthalenesulfonate fluorescence 
  revealed the appearance of hydrophobic binding sites . 
 near - uv cd and 
  proteolysis studies suggested little or no structural alteration outside of 
  the c - terminal region . 
 in contrast to wild type , mt - ftl homopolymers 
  precipitated at much lower iron loading , had a diminished capacity to 
  incorporate iron , and were less thermostable . 
 however , precipitation was 
  significantly reversed by addition of iron chelators both in vitro 
  and in vivo . 
 our results reveal substantial protein conformational 
  changes localized at the 4-fold pore of mt - ftl homopolymers and imply that the 
  c terminus of the mt - ftl polypeptide plays an important role in ferritin 
  solubility , stability , and iron management . 
 we propose that the protrusion of 
  some portion of the c terminus above the spherical shell allows it to 
  cross - link with other mutant polypeptides through iron bridging , leading to 
  enhanced mutant precipitation by iron . 
 our data suggest that hereditary 
  ferritinopathy pathogenesis is likely to result from a combination of 
  reduction in iron storage function and enhanced toxicity associated with 
  iron - induced ferritin aggregates . \\ 
 \midrule 
Model & \small apoferrin is a member of the nuclear receptor superfamily 
  family of membrane proteins. 
 apoferrin is a member of the 
  family of apoferrin family. 
 apoferrin is a member of the 
  family of apoferrin family. 
 apoferrin is a member of the 
  family of apoferrin family. 
 apoferrin is a member of the 
  family of apoferrin family. 
 apoferrin is a member of the 
  family of apoferrin family. 
 apoferrin is a member of the family of \\ 
 \midrule 
Metrics & Rouge1: 13.33, Rouge2: 1.35, RougeL: 12.0, RougeLsum: 12.0, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 25\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny intracellular signaling pathways transmit signals of various extracellular stimuli to their cytosolic and nuclear targets in order to induce biological responses , such as proliferation , differentiation , cell death and migration . 
 when needed , the signals are transmitted from the cytoplasm to the nucleus via translocation of one or more components of each of the signaling pathways involved . 
 thus , after stimulation , a large number of signaling proteins are rapidly translocated to the nucleus to induce and regulate many nuclear processes . 
 however , despite the importance of stimulated nuclear signaling , the mechanisms by which these components reach the nucleus upon stimulation have been elucidated only for a few signaling pathways . 
 classic nuclear shuttling is mediated by an importin- complex that binds to cargoes containing a nuclear localization signal ( nls ) , consisting of mono- or bi - partite clusters of basic amino acids [ 1 - 3 ] . 
 this importin- complex often acts as a housekeeping mechanism that shuttles most nuclear proteins immediately to the nucleus after their translation . 
 the relocalization of cargoes is followed by the dissociation of the proteins from the importins upon binding to rangtp , which exports the importins back to the cytoplasm , while the cargo remains in the nucleus . 
 however , only a limited number of signaling proteins , such as nfb   and erk5 ( extracellular signal - regulated kinase 5 ) [ 8 - 10 ] , use this machinery for their stimulated nuclear shuttle . aside from this canonical mechanism , 
 importin-   or similar karyopherins , termed -like importins , operate by binding to non - canonical nlss to mediate translocation without the assistance of importin-. the mechanism by which these components operate is much less understood and is currently under investigation . recently 
 , several -like importins have been implicated in the stimulated nuclear translocation of signaling proteins . here , 
 we propose that this group of importins might be responsible for the swift nuclear shuttling of many proteins following various stimuli . 
 the rapid and robust activation of erk1/2 allows the phosphorylation and modulation of the activity of more than 300 proteins , which are localized either in the cytoplasm or the nucleus [ 13 - 15 ] . 
 these substrates are important for the induction and regulation of cellular processes , including proliferation , differentiation , and migration amongst others [ 16 - ... \\ 
 \midrule 
Gold & \tiny classic nuclear shuttling is mediated by an importin- heterodimer that binds to cargoes containing a nuclear localization signal , and shuttles most nuclear proteins immediately after their translation . aside from this canonical mechanism , kariopheryn-s or -like importins 
 operate by binding to non - canonical nuclear localization signals to mediate translocation without the assistance of importin-. the mechanism by which these components operate is much less understood and is currently under investigation . recently 
 , several -like importins have been implicated in the stimulated nuclear translocation of signaling proteins . here , 
 we propose that this group of importins might be responsible for the swift nuclear shuttling of many proteins following various stimuli . \\ 
 \midrule 
Model & \small the nuclear translocation signal ( nl ) is a key regulator of many cellular processes, including proliferation, differentiation, cell death, migration, and migration. 
 recent studies have shown that the nuclear translocation signal ( nl ) is required for the induction and regulation of many nuclear processes, including proliferation, differentiation, migration, and migration. here 
, we discuss the role of nl in the regulation of the nuclear translocation signal ( nl ), as well as the mechanisms that regulate it. \\ 
 \midrule 
Metrics & Rouge1: 33.33, Rouge2: 5.0, RougeL: 18.52, RougeLsum: 32.1, Summary length (tokens): 100
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 75\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny helicobacter pylori is a stomach bacterium that colonizes \textasciitilde{}50\% of people globally.1 
 h. pylori is the primary risk factor for gastric cancer  the third highest cause of global cancer morbidity.2 
 h. 
 pylori infection rates are highly dependent on socioeconomic status ; \textasciitilde{}80\% of those living in low socioeconomic areas of latin america , asia , and eastern europe are infected , compared with \textless{} 20\% of asymptomatic caucasians in the usa.3 
 h. pylori infection is treatable with different regimens of antibiotics,4 and eradication of h. pylori is a recognized way to lower incidence of gastric cancer.5 however , recurrence of infection is variable,6,7 and the emergence of antibiotic resistance compromises treatment efficacy . 
 thus , determining the best course of treatment is important to improve treatment efficacy and to reduce recurrence of h. pylori infection . 
 unfortunately , there is no broad consensus about an optimal antibiotic therapy for the treatment of h. pylori . 
 for example , meta - analyses of european and asian clinical data compared the standard triple therapy ( amoxicillin , clarithromycin , and a proton - pump inhibitor for 714 days ) with 5- or 10-day quadruple therapy regimens ( adding metronidazole or tinidazole to the triple therapy ) and found that quadruple therapies are both significantly more effective and cheaper than the triple therapy.810 however , we previously published a study comparing eradication therapies in seven sites of six latin american countries that showed that the 14-day triple therapy was superior to the 5-day concomitant quadruple therapy , and no different than the 10-day sequential quadruple therapy.11,12 these inconsistencies reflect localized differences in antibiotic use practices , such as the use of clarithromycin for upper respiratory infections.13 the differences in efficacy of antibiotic therapy are supported by primary antibiotic resistance data . for example , h. pylori resistance to amoxicillin varied widely between africa ( 65.6\% ) , europe ( 0.5\% ) , asia ( 11.6\% ) , and the americas ( 2.2\%).12 even in the same region , patterns of resistance differ : within central and latin america , reported average metronidazole resistance varies from 30\% in argentina to 83\% in columbia , and tetracycline resistance varies from 2\% in brazil to 33\% in columbia.14 as such , characterizing local resistance patterns is important for selecting therapies with the highest likelihood of success . 
 our research focus... \\ 
 \midrule 
Gold & \tiny objectivesgastric carcinoma is the most common cancer and cause of cancer mortality in peru . 
 helicobacter pylori , a bacterium that colonizes the human stomach , is a group 1 carcinogen due to its causal relationship to gastric carcinoma . while eradication of h. pylori can help prevent gastric cancer , characterizing regional antibiotic resistance patterns 
 is necessary to determine targeted treatment for each region . 
 thus , we examined primary antibiotic resistance in clinical isolates of h. pylori in lima , peru.materials and methodsh . 
 pylori strains were isolated from gastric biopsies of patients with histologically proven h. pylori infection . 
 primary antibiotic resistance among isolates was examined using e - test strips . 
 isolates were examined for the presence of the caga pathogenicity island and the vaca m1/m2 alleles via polymerase chain reaction.resultsseventy-six isolates were recovered from gastric biopsies . 
 clinical isolates showed evidence of antibiotic resistance to 1 ( 27.6\% , n=21/76 ) , 2 ( 28.9\% , n=22/76 ) , or 3 antibiotics ( 40.8\% ) . 
 of 76 isolates , eight ( 10.5\% ) were resistant to amoxicillin and clarithromycin , which are part of the standard triple therapy for h. pylori infection . 
 no trends were seen between the presence of caga , vaca m1 , or vaca m2 and antibiotic resistance.conclusionthe rate of antibiotic resistance among h. pylori isolates in lima , peru , is higher than expected and presents cause for concern . to develop more targeted eradication therapies for h. pylori in peru , more research 
 is needed to better characterize antibiotic resistance among a larger number of clinical isolates prospectively . \\ 
 \midrule 
Model & \small helicobacter pylori infection is the third most common cause of global cancer morbidity. 
 eradication of helicobacter pylori is a recognized way to lower incidence of gastric cancer. 
 however, there is no broad consensus about an optimal antibiotic therapy for the treatment of helicobacter pylori. 
 we assessed primary antibiotic resistance to helicobacter pylori among 76 isolates from a cohort of patients recruited in lima, peru. 
 primary antibiotic resistance to metronidazole, amoxicillin, tetracycline, clarithromycin, levofloxacin, and rifamp \\ 
 \midrule 
Metrics & Rouge1: 50.0, Rouge2: 17.28, RougeL: 32.93, RougeLsum: 47.56, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 95\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny in general , brain injury can occur due to sudden and severe head strike to a hard object , which can be mild , moderate or severe ( 1 ) . 
 the main causes of head injury include traffic accidents , falling from heights , physical violence , accidents at work , inside home accidents and during exercise incidents 
 . however , the most important cause of head trauma in iranian population is traffic accident ( 2 ) . among the warning signs of head trauma are nausea , vomiting , dizziness , headache , blurred vision , and loss of balance , difficulty in sleeping , memory problems , tinnitus and fatigue ( 3 ) . 
 nausea and vomiting are the most common complications after minor head trauma that in addition to severe harassment of patients increases the risk of aspiration and intracranial pressure rising . 
 ondansetron is a serotonin 5-ht3 receptor antagonist , which connects to the peripheral and central receptors of serotonin ( 1 ) . 
 this drug is mostly used in nausea and vomiting after chemotherapy and surgery ( 2 ) . 
 it does not have any effect on dopamine receptors thus ; it does not have extra pyramidal effect ( 3 ) . 
 this drug has a half - life of 2 - 7 hours and is metabolized in the liver where it changes into glucuronide and sulfate which is inactive . 
 its most common side effects include headaches , fatigue , diarrhea , constipation , dizziness and anxiety . 
 the recommended dose for the treatment of nausea and vomiting is 4 - 8 milligrams ( 4 , 5 ) . 
 metoclopramide as an old antiemetic is mostly used in high doses , before chemotherapy and for nausea and vomiting caused by various reasons ( 6 - 8 ) . 
 this drug blocks the dopamine receptors on the peripheral and central dopamine receptors and increases the movement of the upper gastrointestinal tract without increasing secretion ( 9 , 10 ) . 
 its intravenous absorption takes about 3 minutes and the peak of its effect is about 15 minute . 
 this drug is metabolized in the liver and its half - life is approximately 4 - 5 hours ( 11 ) . 
 its most common side effects include dystonia \textless{} 10\% , fatigue , drowsiness , and flushing . 
 based on the above - mentioned reasons , the present study was aimed to compare the antiemetic effects of metoclopramide and ondansetron in the treatment of post head trauma nausea and vomiting . 
 study design and setting 
  the study was a controlled , randomized , double blind clinical trial , which was conducted in the first 6 months of 2014 in al - zahra a... \\ 
 \midrule 
Gold & \tiny introduction : nausea and vomiting are the most common complications after minor head trauma that increases the risk of intracranial pressure rising . therefore , the present study was aimed to compare the antiemetic effects of metoclopramide and ondansetron in the treatment of post - traumatic nausea and vomiting . methods : the study was a controlled , randomized , double blind clinical trial , which was conducted in the first 6 months of 2014 in emergency department al - zahra and kashani hospitals in isfahan , iran . the patients with minor head trauma associated with nausea and vomiting were randomly divided into 2 groups : treatment with metoclopramide ( 10mg/2ml , slow injection ) and treatment with ondansetron ( 4mg/2ml , slow injection ) . 
 the comparison between the 2 groups was done regarding antiemetic efficacy and side effects using spss 21 statistical software . 
 results:120 patients with minor head trauma were distributed and studied into two groups of 60 patients ( mean age 35.614.1 years ; 50.0\% male ) . 
 administration of both ondansetron and metoclopramide significantly reduced the severity of nausea ( p\textless{}0.001 ) . 
 changes in the severity of nausea in both groups before and after the treatment revealed that nausea had been decreased significantly in both groups ( p \textless{} 0.001 ) . 
 the incidence of fatigue ( p=0.44 ) , headache ( p=0.58 ) and dystonia ( p=0.06 ) had no significant difference in the two groups but the incidence of drowsiness and anxiety in the metoclopramide group was significantly higher ( p \textless{} 0.001 ) . 
 conclusion : the present study indicated that the treatment effectiveness of ondansetron and metoclopramide are similar . 
 however , incidence of drowsiness and anxiety in the metoclopramide was considerably higher . since these complications can have adverse effects on the treatment of patients with brain injury , it is suggested that it may be better to use ondansetron in these patients . \\ 
 \midrule 
Model & \small background : head injury can occur due to sudden and severe head strike to a hard object, which can be mild, moderate or severe. 
 metoclopramide as an old antiemetic is mostly used in high doses, before chemotherapy and for nausea and vomiting caused by various reasons. 
 the present study was aimed to compare the antiemetic effects of metoclopramide and ondansetron in the treatment of post head trauma nausea and vomiting. 
 methods : this randomized, double blind clinical trial was conducted in the first 6 months of 2014 in isfahan, iran. 
 the patients were randomly divided into \\ 
 \midrule 
Metrics & Rouge1: 59.69, Rouge2: 46.56, RougeL: 51.31, RougeLsum: 58.64, Summary length (tokens): 129
 \\ 

    \bottomrule
    \end{tabular}
}
\caption{Examples of the PubMed dataset using the model pubmed-1024-128_base_diverse}
\label{tab:examples_pubmed-1024-128_base_diverse}
\end{table*}


==> summaries/pubmed-1024-128_small_diverse.tex <==

\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
    \begin{tabular}{ l p{21cm} }
    \toprule
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 5\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny in the last decade the amount of data regarding micrornas ( mirs ) and their target genes described in the literature has expanded tremendously . 
 the volume of information on this new group of regulators ( i.e. , mirs ) has complicated attempts to integrate this data within existing metabolic and signalling networks . as regulators of gene expression 
 in addition , a single mir can potentially regulate multiple different genes at the same time , leading to complex functional outcomes . 
 however , from another perspective , the identification of groups of genes targeted by the same mir and the clustering of these genes within individual signalling pathways represents a means to understand the cross talk between multiple signalling networks and their role in a common biological process . 
 the focus of this review is to summarize the validated groups of mirs functionally linked to the cross talk between tgf- , notch , and wnt signalling during the common biological process of epithelial - to - mesenchymal transition ( emt ) . in particular 
 , this review will address whether the documented cross talk between these three important emt - associated pathways could be further reinforced by the identification of a  signature  of mirs , already depicted in the literature but not yet  sharpened  or clearly defined in this role . in the past years , many studies have elegantly described the role of tgf- , notch , and wnt pathways in promoting emt and emt - associated disorders including fibrosis and metastatic dissemination in cancer [ 16 ] . here 
 we identify published and validated interactions between mirs and genes involved in tgf- , notch , and wnt signalling . 
 this led to the discovery of a signature of 30 mirs each regulating all three pathways . 
 we then searched for additional validated genes targeted by these 30 mirs and then further clustered these into the tgf- , notch , and wnt signalling pathways . 
 interestingly , in our attempt to identify mirs that were common to all three of these signalling pathways , we found that the 30-mir signature strongly reinforced existing evidence supporting cross talk between these three pathways during emt . 
 in this review we used tarbase v6.0 , the largest currently available manually curated mir target gene database , which includes targets derived from specific and high throughput experiments . using tarbase v6.0 we searched the collection of manually curated , 
 experimentally validated mir - gene intera... \\ 
 \midrule 
Gold & \tiny epithelial - to - mesenchymal transition ( emt ) is a reversible process by which cancer cells can switch from a sessile epithelial phenotype to an invasive mesenchymal state . 
 emt enables tumor cells to become invasive , intravasate , survive in the circulation , extravasate , and colonize distant sites . 
 paracrine heterotypic stroma - derived signals as well as paracrine homotypic or autocrine signals can mediate oncogenic emt and contribute to the acquisition of stem / progenitor cell properties , expansion of cancer stem cells , development of therapy resistance , and often lethal metastatic disease . 
 emt is regulated by a variety of stimuli that trigger specific intracellular signalling pathways . 
 altered microrna ( mir ) expression and perturbed signalling pathways have been associated with epithelial plasticity , including oncogenic emt . in this review 
 we analyse and describe the interaction between experimentally validated mirs and their target genes in tgf- , notch , and wnt signalling pathways . 
 interestingly , in this process , we identified a  signature  of 30 experimentally validated mirs and a cluster of validated target genes that seem to mediate the cross talk between tgf- , notch , and wnt signalling networks during emt and reinforce their connection to the regulation of epithelial plasticity in health and disease . \\ 
 \midrule 
Model & \small micrornas ( mirs ) are a class of small noncoding rnas that regulate multiple gene expression at the same time, leading to complex functional outcomes. 
 recent studies have shown that mirs regulate multiple different pathways at the same time, leading to complex functional outcomes. 
 however, from another perspective, the identification of genes targeted by the same mir and the clustering of these genes within individual signalling pathways represents a means to understand the cross talk between multiple signalling pathways and their role in a common biological process. in this review 
, we summarize the published studies of mir-, notch, and wnt signalling in \\ 
 \midrule 
Metrics & Rouge1: 20.22, Rouge2: 0.0, RougeL: 11.24, RougeLsum: 14.61, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Bottom 25\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny mhc class ii molecules are heterodimeric cell surface glycoproteins that bind exogenously derived antigenic peptides and present them to cd4 t cells 12 . class ii  and  chains 
 are translocated into the endoplasmic reticulum ( er ) , where they form nonamers with invariant ( ii ) chain 3 . 
 ii chain prevents the binding of immunogenic peptides due to the presence of a 14amino acid domain ( clip ) that occupies the peptide - binding groove of / dimers 3 . after ii degradation in the endocytic pathway , the mhc - encoded molecules hla - dm ( or h2-m in the mouse ) and hla - do ( h2-o ) facilitate the removal of clip from / dimers , allowing peptide binding 456 . 
 ii chain has been implicated in functions such as er export , endosome targeting , and even b cell maturation 37 . 
 two alternatively spliced ii isoforms exist ( p31 and p41 ) , distinguished by a 64-residue domain in the lumenal portion of p41 8 . 
 the isoforms are expressed differently in various apcs and regulate the presentation of certain antigen epitopes in b cells 9 . 
 this difference may reflect protease inhibition by the amino acid insertion in p41 , as it has been shown to inhibit the lysosomal cysteine protease cathepsin l both in vitro and in vivo 910 . 
 therefore , ii chain may contribute to the modulation of the proteolysis in the endocytic pathway and thus modulate antigen processing indirectly 1112 . 
 we demonstrate here that ii chain deletion leads to the lysosomal degradation of h2-mb in apcs , suggesting that ii chain is required to prevent the proteolysis of h2-m and perhaps of other proteins 
 . this feature may help explain how ii chain expression affects t cell selection and b cell maturation independently from its effect on mhc class ii traffic 131415 . 
 c57bl/6 ( control ) and ii , ii p31 1416 , class ii , and class ii / ii mice ( the gift of p. marrack , university of colorado health sciences center , denver , co ) were kept in a pathogen - free environment for 78 wk before killing . 
 splenocytes were obtained as described 7 . bone marrow  derived dendritic cells ( dcs ) were cultured as described 17 . 
 after purification , immature dcs were characterized by immunofluorescence and processed in parallel with the lps - treated dcs . 
 the primers used here to detect i - a  , h2-m , and h2-m are identical to the primers described previously 19 . 
 3  10 late dcs were pulse labeled with 7.5 mci / ml of [ s]methionine translabel ( icn ) and chased as described 17 . 
 ... \\ 
 \midrule 
Gold & \tiny the association of invariant ( ii ) chain with major histocompatibility complex ( mhc ) class ii dimers is required for proper antigen presentation to t cells by antigen - presenting cells . 
 mice lacking ii chain have severe abnormalities in class ii transport , t cell selection , and b cell maturation . 
 we demonstrate here that h2-m , which is required for efficient class ii antigenic peptide loading , is unexpectedly downregulated in splenocytes and mature dendritic cells ( dcs ) from ii/ mice . 
 downregulation reflects an increased rate of degradation in ii/ cells 
 . degradation apparently occurs within lysosomes , as it is prevented by cysteine protease inhibitors such as e64 , but not by the proteasome inhibitor lactacystin . 
 thus , ii chain may act as a lysosomal protease inhibitor in b cells and dcs , with its deletion contributing indirectly to the loss of h2-m . \\ 
 \midrule 
Model & \small mhc class ii molecules are heterodimeric cell surface glycoproteins that bind exogenously derived antigenic peptides and present them to cd4 t cells 12. 
 type ii chains are translocated into the endoplasmic reticulum ( er ), where they form nonamers with invariant ( ii ) chain 3. 
 type ii chains are translocated into the endoplasmic reticulum ( er ), where they form nonamers with invariant ( ii ) chain 3. 
 type ii chains are translocated into the endoplasmic reticulum ( er ), where \\ 
 \midrule 
Metrics & Rouge1: 27.67, Rouge2: 8.92, RougeL: 17.61, RougeLsum: 25.16, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 75\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny stroke , after myocardial infarction ( mi ) , is the second leading reason for mortality in iran as with many countries worldwide . 
 the epidemiology of stroke has already been investigated in the american , european , african , and asian countries . 
 no comprehensive study has yet investigated the epidemiology of stroke , particularly in mi patients , in iran , one of the largest countries in southwest asia . 
 stroke and mi share many risk factors , most prevalent of which are smoking , dyslipidemia , type 2 diabetes , and hypertension . 
 the risk factors for stroke and mi , especially smoking , hypertension , and dyslipidemia are highly prevalent in iran , as well . according to projections 
 urbanism , increased life expectancy , reduction in childbirth , aging and elderly population , epidemiological changes , socioeconomic status , geographical conditions , and lifestyles such as poor diet , stress , and low mobility are the main causes of the burden of noncommunicable diseases , particularly stroke . because the determinants of stroke in different communities are various , we require knowledge about the risk factors and determinants of mortality in a community for effective planning and selection of appropriate strategies for the prevention and management of stroke and heart attack as the most important causes of death . since no comprehensive study has yet been investigated the status and mortality determinants of stroke in mi patients in iran , this study is conducted to determine and compare the determinants of mortality due to stroke in mi patients . 
 in this retrospective cohort study , the data obtained from the mi registry of iran 's cardiovascular diseases surveillance system were analyzed . around 
 20,750 hospitalized patients with mi with a new presentation ( hospitalized in 540 hospitals ) between april , 2012 and march , 2013 were enrolled . 
 the study was approved by the management center of noncommunicable diseases and the department of cardiovascular diseases prevention of iran 's ministry of health and medical education ( approval no . 
 the research followed the principles of the declaration of helsinki ; the researchers did not conduct any interventions on the patients , and an institutional review board approved this research . 
 the study protocol was approved by an independent scientific review committee ( at shahid beheshti university medical of sciences ) ( no . 
 inclusion criteria were determined according to the world... \\ 
 \midrule 
Gold & \tiny background : the data and determinants of mortality due to stroke in myocardial infarction ( mi ) patients are unknown . 
 this study was conducted to evaluate the differences in risk factors for hospital mortality among mi patients with and without stroke history.materials and methods : this study was a retrospective , cohort study ; 20,750 new patients with mi from april , 2012 to march , 2013 were followed up and their data were analyzed according to having or not having the stroke history . 
 stroke and mi were defined based on the world health organization 's definition . 
 the data were analyzed by logistic regression in stata software.results:of the 20,750 studied patients , 4293 had stroke history . 
 the prevalence of stroke in the studied population was derived 20.96\% ( confidence interval [ ci ] 95\% : 20.1321.24 ) . of the patients , 2537 ( 59.1\% ) had st - elevation mi ( stemi ) . 
 mortality ratio in patients with and without stroke was obtained 18.8\% and 10.3\% , respectively . 
 the prevalence of risk factors in mi patients with and without a stroke is various . 
 the adjusted odds ratio of mortality in patients with stroke history was derived 7.02 ( 95\% ci : 5.429 ) for chest pain resistant to treatment , 2.39 ( 95\% ci : 1.972.9 ) for stemi , 3.02 ( 95\% ci : 2.53.64 ) for lack of thrombolytic therapy , 2.2 ( 95\% ci : 1.662.91 ) for heart failure , and 2.17 ( 95\% ci : 1.62.9 ) for ventricular tachycardia.conclusion:with regards to the factors associated with mortality in this study , it is particularly necessary to control the mortality in mi patients with stroke history . 
 more emphasis should be placed on the mi patients with the previous stroke over those without in the interventions developed for prevention and treatment , and for the prevention of avoidable mortalities . \\ 
 \midrule 
Model & \small background : stroke and myocardial infarction ( mi ) share many risk factors, most prevalent of which are smoking, dyslipidemia, type 2 diabetes, and hypertension. 
 the aim of this study was to determine and compare the determinants of stroke in mi patients.methods:in this retrospective cohort study, the data obtained from the mi registry of iran's cardiovascular diseases surveillance system were analyzed. 
 patients with mi were defined by the date at mi diagnosis, hospital stay, and follow - up till discharge or death ( outcome ). 
 odds ratio ( or ) of mortality for clinical and demographic risk factors were calculated by logistic regression.results \\ 
 \midrule 
Metrics & Rouge1: 55.88, Rouge2: 20.79, RougeL: 31.37, RougeLsum: 51.96, Summary length (tokens): 129
 \\ 
\\ 
 \midrule 
\multicolumn{2}{l}{Top 95\% example (Sorted by rougeL)}\\ 
 \midrule 
Document & \tiny stroke commonly causes loss of motor function due to weakening of upper / lower extremity 
 muscles1 . according to ryerson2 , 
 use the affected upper extremity decreases 
 because of the patient s dependency on the unaffected upper extremity for normal functions , 
 which results in problems such as learned disuse , asymmetric postural patterns , 
 contractures , and aggravated functional restrictions involving the affected upper extremity . 
 therefore , to improve functions of the affected upper extremity in stroke patients , measures 
 that maximize opportunities to use the affectedupper extremity are necessary . 
 bilateral 
 activities have been discussed as measures to improve the body symmetry and to reduce 
 abnormal muscle tone3 , thereby promoting 
 voluntary movement of the affected upper extremity4 . thus far , bilateral upper extremity coordination movements have 
 been applied in the form of bilateral single exercises utilizing tasks such as figure 
 imitation5 , robot arm upper extremity 
 mechanisms6 and functional 
 stretching7 , and bilateral complex 
 exercises combined with the principle of motor learning , such as rhythmic acoustic8 , unaffected extremity weight addition9 , and active neuromuscular electrical 
 stimulation in stroke patients10 . 
 most 
 previous studies have reported the positive effects of these exercises on motor function 
 recovery in stroke patients . 
 whitall et al.8 reported that when chronic hemiplegia patients underwent bilateral 
 training to push and pull upper extremity apparatuses , including acoustic signals , their 
 upper extremity functions were improved . in a study conducted by summer et al.7 with 12 chronic stroke patients , 
 the 
 movement time of the patients affected side upper extremity decreased and upper extremity 
 functions showed more improvement when they performed tasks to hold objects by stretching 
 both hands simultaneously then when they performed tasks to hold objects by stretching only 
 one hand . 
 however , lee su - jin11 advised 
 that the tasks in those studies involved mostly gross motor exercises of the upper extremity 
 and simple repetitive training tasks , and that they were not sufficient to improve patients 
 grasping ability to hold objects with various sizes , shapes , and weights using the shoulder , 
 elbow , wrist , and fingers . 
 although studies that applied diverse functional training tasks including activities of 
 daily living to symmetric bilateral upper ... \\ 
 \midrule 
Gold & \tiny [ purpose ] the purpose of this study was to investigate the effects of task - oriented 
 bilateral arm training and repetitive bilateral arm training on upper limb function and 
 activities of daily living in stroke patients . 
 [ subjects ] forty patients with hemiplegia 
 resulting from stroke were divided into a task orientied bilateral arm training group 
 ( n=20 ) and a repetitive bilateral arm training group ( n=20 ) . 
 [ methods ] the task - oriented 
 group underwent bilateral arm training with 5 functional tasks , and the repetitive group 
 underwent bilateral arm training with rhythmin auditory cueing for 30 minutes / day , 5 
 times / week , for 12 weeks . 
 [ results ] the upper limb function and the ability to perform 
 activities of daily living improved significantly in both groups . 
 although there were 
 significant differences between the groups , the task - oriented group showed greater 
 improvement in upper limb function and activities of daily living . 
 [ conclusion ] we 
 recommend bilateral arm training as well as adding functional task training as a clinical 
 intervention to improve upper limb function activities of daily living in patients with 
 hemiplegia . \\ 
 \midrule 
Model & \small [ purpose ] the purpose of this study was to compare the effects of symmetric bilateral upper 
 extremity exercises using diverse functional training tasks with the effects of repetitive 
 bilateral upper extremity exercises including acoustic signals on the recovery of upper extremity function and daily 
 living activities in stroke paitents. 
 [ subjects and methods ] forty 
 patients with hemiplegia resulting from stroke were randomly and equally 
 assigned to a task - oriented bilateral arm training group ( tbg : 11 
 males, 9 females ) and a repetitive bilateral arm training group ( rbg : 13 males, 7 
 females ). 
 both groups performed their exercises for \\ 
 \midrule 
Metrics & Rouge1: 62.03, Rouge2: 34.59, RougeL: 50.27, RougeLsum: 60.96, Summary length (tokens): 129
 \\ 

    \bottomrule
    \end{tabular}
}
\caption{Examples of the PubMed dataset using the model pubmed-1024-128_small_diverse}
\label{tab:examples_pubmed-1024-128_small_diverse}
\end{table*}

